OdysseyArena: Benchmarking Large Language Models For Long-Horizon, Active and Inductive Interactions

The advancement of Large Language Models (LLMs) has catalyzed the development of autonomous agents capable of navigating complex environments. However, existing evaluations primarily adopt a deductive paradigm, where agents execute tasks based on explicitly provided rules and static goals, often within limited planning horizons. Crucially, this neglects the inductive necessity for agents to discover latent transition laws from experience autonomously, which is the cornerstone for enabling agentic foresight and sustaining strategic coherence. To bridge this gap, we introduce OdysseyArena, which re-centers agent evaluation on long-horizon, active, and inductive interactions. We formalize and instantiate four primitives, translating abstract transition dynamics into concrete interactive environments. Building upon this, we establish OdysseyArena-Lite for standardized benchmarking, providing a set of 120 tasks to measure an agent's inductive efficiency and long-horizon discovery. Pushing further, we introduce OdysseyArena-Challenge to stress-test agent stability across extreme interaction horizons (e.g., > 200 steps). Extensive experiments on 15+ leading LLMs reveal that even frontier models exhibit a deficiency in inductive scenarios, identifying a critical bottleneck in the pursuit of autonomous discovery in complex environments. Project homepage: https://os-copilot.github.io/OdysseyArena-Home/

==> Tables/comparison.tex <==


\begin{table}[t]
\centering
\caption{Comparison of representative multi-turn agentic benchmarks. \emph{Ind.} indicates whether inductive reasoning is required. \emph{Horizon} denotes the number of steps required to complete a task, categorized as short ($<$50), long (50–100), or X-Long ($>$100). \emph{Deploy} describes the evaluation setup required to run the environment, with API-based deployment being the most lightweight.}
\label{tab:agent_benchmark_comparison}
\begin{tabular}{lccc}
\toprule
Benchmark 
% & Env.
& Ind.
% & \# Tasks 
& Horizon
& Deploy
\\
\midrule

% Sokoban
% & \checkmark
% & \xmark
% % & 1
% & Long
% & Simulator
% \\

% Tower of Hanoi
% % & \checkmark
% & \xmark
% % & 1
% & Finite
% & Simulator
% \\
% % ~\citeyearpar{chollet2026arcagi2newchallengefrontier}
% ARC-AGI-2~\citeyearpar{chollet2026arcagi2newchallengefrontier}
% % & \xmark
% & \checkmark
% % & Large
% & Short
% % & Offline Dataset
% & -
% \\

% Game of 24
% % & \xmark
% & \xmark
% % & 1
% & Short
% % & Symbolic Search
% & -
% \\

% \midrule

% ~\citeyearpar{chevalierbabyai}
BabyAI~\citeyearpar{chevalierbabyai}
% & \checkmark
& \color{checkmarkgreen}\checkmark
% & Finite
& Long
& Simulator
\\
% ~\citeyearpar{shridharalfworld}
ALFWorld~\citeyearpar{shridharalfworld}
% & \checkmark
& \color{checkmarkgreen}\checkmark
% & Finite
& Short
& Simulator
\\

GAIA~\citeyearpar{mialon2023gaia}
&\color{red}\xmark
% & \checkmark
% & Finite
& Long
& Offline
\\

% SWE-bench~\citeyearpar{Jimenez2023SWEbenchCL}
% % & \checkmark
% & \color{red}\xmark
% % & Large
% & Long
% % & Desktop (Dockerized)
% & Docker
% \\

% ~\citeyearpar{zhouwebarena}
WebArena~\citeyearpar{zhouwebarena}
% & \checkmark
& \color{red}\xmark
% & Large
& Short
% & Browser (Dockerized)
& Docker
\\
% ~\citeyearpar{rawlesandroidworld}

% ~\citeyearpar{xie2024osworld}
OSWorld~\citeyearpar{xie2024osworld}
% & \checkmark
& \color{red}\xmark
% & Large
& Long
% & Full OS (Dockerized)
& Docker
\\

AndroidWorld~\citeyearpar{rawlesandroidworld}
% & \checkmark
& \color{red}\xmark
% & Large
& Short
% & Mobile OS (Emulator)
& Emulator
\\



% ~\citeyearpar{wei2025browsecomp}
BrowseComp~\citeyearpar{wei2025browsecomp}
% & \checkmark
& \color{red}\xmark
% & Large
& Long 
% & Full OS (Dockerized)
& API
\\


\midrule
\textbf{\odyssey}
% & \checkmark
& \textbf{\color{checkmarkgreen}\checkmark}
% & $\infty$
& X-Long
& API
% & Native Execution
\\

\bottomrule
\end{tabular}
\end{table}


==> Tables/error_type.tex <==
\begin{table}[htbp]
  \centering
  \caption{Error Categories of Long-Horizon Failures in Gemini 3 Pro Preview (Based on 47 manually analyzed trajectories)}
  \label{tab:error_types}
  \begin{tabular}{l c p{5cm} p{4cm}}
    \toprule
    \textbf{Error Category} & \textbf{Count} & \textbf{Description} & \textbf{Example Failure Trajectory} \\
    \midrule
    Exploration Limitations & 18 & Inability to sufficiently explore the state space or test alternative strategies, leading to entrapment in suboptimal solutions. & The agent cycles through the same ineffective action sequence without exploring novel paths that could achieve the goal. \\
    Memory Limitations & 15 & Failure to retain or retrieve critical historical information from earlier trajectory steps, causing inconsistent decision-making. & The agent forgets a key constraint identified at the task onset and takes an action that violates it, undoing prior progress. \\
    Adaptation Limitations & 10 & Inability to dynamically adjust the policy using environmental feedback (e.g., rewards, state transitions). & Despite repeated negative feedback for a specific action type, the agent persists in selecting similar actions in subsequent steps. \\
    Perceptual Misinterpretation & 4 & Incorrect processing or understanding of sensory inputs, leading to flawed state representations. & The agent misclassifies an object in the environment, resulting in a sequence of actions tailored to the wrong object. \\
    \midrule
    \textbf{Total} & \textbf{47} & \multicolumn{2}{l}{} \\
    \bottomrule
  \end{tabular}
\end{table}
